Landscape of standing variation for tandem duplications in Drosophila yakuba and Drosophila simulans

We have used whole genome paired-end Illumina sequence data to identify tandem duplications in 20 isofemale lines of D. yakuba, and 20 isofemale lines of D. simulans and performed genome wide validation with PacBio long molecule sequencing. We identify 1,415 tandem duplications that are segregating in D. yakuba as well as 975 duplications in D. simulans, indicating greater variation in D. yakuba. Additionally, we observe high rates of secondary deletions at duplicated sites, with 8% of duplicated sites in D. simulans and 17% of sites in D. yakuba modified with deletions. These secondary deletions are consistent with the action of the large loop mismatch repair system acting to remove polymorphic tandem duplication, resulting in rapid dynamics of gain and loss in duplicated alleles and a richer substrate of genetic novelty than has been previously reported. Most duplications are present in only single strains, suggesting deleterious impacts are common. D. simulans shows larger numbers of whole gene duplications in comparison to larger proportions of gene fragments in D. yakuba. D. simulans displays an excess of high frequency variants on the X chromosome, consistent with adaptive evolution through duplications on the D. simulans X or demographic forces driving duplicates to high frequency. We identify 78 chimeric genes in D. yakuba and 38 chimeric genes in D. simulans, as well as 143 cases of recruited non-coding sequence in D. yakuba and 96 in D. simulans, in agreement with rates of chimeric gene origination in D. melanogaster. Together, these results suggest that tandem duplications often result in complex variation beyond whole gene duplications that offers a rich substrate of standing variation that is likely to contribute both to detrimental phenotypes and disease, as well as to adaptive evolutionary change.

==> CoverageCorrelation.tex <==
\begin{figure}[h]
\begin{center}

\includegraphics[scale=0.70]{CovCorr.pdf}

\label{CovCov}
\caption{Number of variants vs. coverage by line in \Dyak {} (A) and \Dsim {} (B).  Regression line (blue) and 95\% CI (grey) are shown. Correlation between coverage and number of duplications is low (\Dyak {} adjusted $R^2=0.21$, \Dsim {} adjusted $R^2=0.03$). }
\end{center}

\end{figure}



==> PacBioTable.tex <==

\begin{center}
\begin{threeparttable}
\caption{Pac Bio Confirmations for line CY17C}
\tiny
\begin{tabular}{cccc}
Chromosome & Start & Stop & Confirmed \\
\hline
0 & 10164056 & 10164577 & Yes \\
0 & 10204361 & 10204494 & Yes \\
0 & 11082344 & 11085513 & Yes \\
0 & 11454199 & 11454798 & Yes \\
0 & 11791812 & 11792896 & Yes \\
0 & 12231658 & 12238883 & Yes \\
0 & 12544338 & 12544932 & Yes \\
0 & 12596845 & 12597053 & Yes \\
0 & 12894471 & 12894671 & Yes \\
0 & 13521555 & 13522843 & Yes \\
0 & 13768117 & 13768370 & Yes \\
0 & 14172239 & 14172458 & No \\
0 & 1434187 & 1435491 & Yes \\
0 & 153714 & 155228 & No \\
0 & 15944998 & 15948170 & Yes \\
0 & 16264723 & 16284646 & Yes \\
0 & 1631349 & 1632283 & Yes \\
0 & 16414309 & 16416275 & Yes \\
0 & 16689283 & 16690706 & Yes \\
0 & 17077700 & 17078693 & Yes \\
0 & 18741929 & 18746697 & Yes \\
0 & 22160922 & 22173382 & Yes \\
0 & 23153724 & 23162933 & Yes \\
0 & 2397145 & 2400994 & Yes \\
0 & 2540641 & 2541141 & Yes \\
0 & 30811 & 31109 & Yes \\
0 & 3177872 & 3189471 & Yes \\
0 & 3185710 & 3196869 & Yes \\
0 & 5038513 & 5043130 & Yes \\
0 & 53912 & 54140 & Yes \\
0 & 6617562 & 6618756 & Yes \\
0 & 6853202 & 6857398 & Yes \\
0 & 7665669 & 7670924 & Yes \\
0 & 7937194 & 7937319 & Yes \\
0 & 8280380 & 8281789 & Yes \\
0 & 833632 & 833787 & Yes \\
0 & 8344311 & 8344720 & Yes \\
0 & 9935517 & 9935759 & Yes \\
1 & 10344910 & 10345378 & Yes \\
1 & 10348256 & 10350937 & Yes \\
1 & 1051430 & 1053425 & Yes \\
1 & 10585970 & 10587591 & Yes \\
1 & 10873174 & 10876328 & Yes \\
1 & 11412985 & 11416198 & Yes \\
1 & 11531806 & 11532092 & Yes \\
1 & 11616544 & 11627893 & Yes \\
1 & 11870953 & 11872819 & Yes \\
1 & 1198204 & 1198587 & Yes \\
1 & 12578204 & 12578940 & Yes \\
1 & 12589873 & 12593820 & Yes \\
1 & 13310476 & 13311857 & Yes \\
1 & 14056332 & 14056966 & Yes \\
1 & 14060197 & 14065508 & Yes \\
1 & 15377363 & 15379792 & Yes \\
1 & 16333002 & 16336287 & Yes \\
1 & 16475111 & 16476986 & Yes \\
1 & 16627714 & 16628834 & Yes \\
1 & 16969317 & 16969672 & Yes \\
1 & 16977546 & 16977980 & Yes \\
1 & 17477743 & 17483758 & Yes \\
1 & 17480309 & 17480964 & Yes \\
1 & 192491 & 193591 & Yes \\
1 & 20650681 & 20651896 & Yes \\
1 & 20851838 & 20856752 & Yes \\
1 & 20867709 & 20868709 & Yes \\
1 & 20994430 & 20995784 & Yes \\
1 & 21051596 & 21051807 & Yes \\
1 & 21888859 & 21890541 & Yes \\
1 & 21956133 & 21970142 & Yes \\
1 & 22142495 & 22143242 & Yes \\
1 & 22229672 & 22240590 & Yes \\
1 & 3639179 & 3642391 & Yes \\
1 & 3688301 & 3689997 & Yes \\
1 & 3748543 & 3748779 & Yes \\
1 & 4351735 & 4352527 & Yes \\
1 & 4507624 & 4509111 & Yes \\
1 & 4561989 & 4563943 & Yes \\
1 & 5026261 & 5027602 & No \\
1 & 7051842 & 7052051 & Yes \\
2 & 10699218 & 10701733 & Yes \\
2 & 10705351 & 10711729 & Yes \\
2 & 11199268 & 11201983 & Yes \\
2 & 11522584 & 11523299 & Yes \\
2 & 11551259 & 11554075 & Yes \\
2 & 1192252 & 1198186 & Yes \\
2 & 12091221 & 12095128 & Yes \\
2 & 1234222 & 1235055 & Yes \\
2 & 126303 & 128688 & Yes \\
2 & 1267547 & 1269515 & Yes \\
2 & 12873611 & 12874020 & Yes \\
2 & 1298866 & 1302456 & Yes \\
2 & 140351 & 143625 & Yes \\
2 & 14915735 & 14922064 & Yes \\
2 & 14916089 & 14925568 & Yes \\
2 & 14921170 & 14923118 & Yes \\
2 & 15320662 & 15324437 & Yes \\
2 & 15591344 & 15591787 & Yes \\
2 & 15595900 & 15596602 & Yes \\
2 & 16915401 & 16922730 & Yes \\
2 & 17014060 & 17017680 & Yes \\
2 & 17712761 & 17713480 & Yes \\
2 & 17738259 & 17744715 & Yes \\
2 & 17738426 & 17739224 & Yes \\
2 & 17742992 & 17744704 & Yes \\
2 & 18128177 & 18128325 & Yes \\
2 & 18340872 & 18341767 & Yes \\
2 & 19236665 & 19238004 & Yes \\
2 & 19575981 & 19576340 & Yes \\
2 & 1978655 & 1980831 & Yes \\
2 & 1978794 & 1978911 & Yes \\
2 & 20331116 & 20331457 & Yes \\
2 & 20346896 & 20349545 & Yes \\
2 & 20384228 & 20385080 & Yes \\
2 & 20556535 & 20557016 & Yes \\
2 & 20876827 & 20877288 & Yes \\
2 & 231409 & 236136 & Yes \\
2 & 2456185 & 2468412 & Yes \\
2 & 261487 & 266019 & Yes \\
2 & 2621213 & 2625329 & Yes \\
2 & 292319 & 294519 & Yes \\
2 & 312743 & 315531 & Yes \\
2 & 314045 & 314339 & Yes \\
2 & 3639973 & 3644389 & Yes \\
2 & 3686554 & 3691429 & Yes \\
2 & 414713 & 418549 & Yes \\
2 & 4606870 & 4621168 & Yes \\
2 & 543979 & 547207 & Yes \\
2 & 550564 & 555698 & Yes \\
2 & 568027 & 572649 & Yes \\
2 & 5933375 & 5933612 & No \\
2 & 60107 & 68217 & Yes \\
2 & 6275581 & 6278705 & Yes \\
2 & 6750316 & 6750822 & Yes \\
2 & 6888816 & 6889491 & Yes \\
2 & 6949028 & 6949167 & Yes \\
2 & 6990941 & 6992414 & Yes \\
2 & 7085103 & 7088180 & Yes \\
2 & 7488837 & 7490999 & Yes \\
2 & 7499905 & 7500222 & Yes \\
2 & 8218637 & 8220875 & Yes \\
2 & 8627195 & 8631730 & Yes \\
2 & 8628288 & 8637097 & Yes \\
2 & 8660527 & 8664855 & Yes \\
2 & 8693878 & 8697950 & Yes \\
2 & 901994 & 911580 & Yes \\
2 & 9395796 & 9395876 & Yes \\
2 & 9568935 & 9569008 & Yes \\
2 & 9576108 & 9579788 & Yes \\
2 & 9718894 & 9722579 & Yes \\
3 & 10097943 & 10098401 & Yes \\
3 & 10460172 & 10460672 & Yes \\
3 & 10486354 & 10487155 & Yes \\
3 & 10796998 & 10797687 & Yes \\
3 & 11367086 & 11367592 & Yes \\
3 & 12616185 & 12616299 & Yes \\
3 & 12994638 & 12995090 & Yes \\
3 & 14420131 & 14420863 & Yes \\
3 & 14759218 & 14759582 & Yes \\
3 & 15375448 & 15375633 & No \\
3 & 15709614 & 15709783 & Yes \\
3 & 15977640 & 15977783 & Yes \\
3 & 1616894 & 1617449 & Yes \\
3 & 16990151 & 16990245 & Yes \\
3 & 17669144 & 17670186 & Yes \\
3 & 18175136 & 18177496 & Yes \\
3 & 18218525 & 18219473 & Yes \\
3 & 18564946 & 18568426 & Yes \\
3 & 18729973 & 18730230 & Yes \\
3 & 18804671 & 18805512 & Yes \\
3 & 18808010 & 18808880 & Yes \\
3 & 19744296 & 19744448 & Yes \\
3 & 19810217 & 19810349 & Yes \\
3 & 19859038 & 19866130 & Yes \\
3 & 20188603 & 20189100 & Yes \\
3 & 20640778 & 20646886 & Yes \\
3 & 20651169 & 20654842 & Yes \\
3 & 20761443 & 20768078 & Yes \\
3 & 2094815 & 2098815 & Yes \\
3 & 21252134 & 21270342 & Yes \\
3 & 2140691 & 2142534 & No \\
3 & 2263061 & 2263383 & Yes \\
3 & 254858 & 255317 & Yes \\
3 & 3108853 & 3131554 & Yes \\
3 & 3623232 & 3623498 & Yes \\
3 & 5168928 & 5171821 & Yes \\
3 & 6027171 & 6028326 & Yes \\
3 & 6034154 & 6034546 & Yes \\
3 & 6979162 & 6979796 & Yes \\
3 & 804465 & 805608 & Yes \\
3 & 8277294 & 8278561 & Yes \\
3 & 8318145 & 8319291 & Yes \\
3 & 8487649 & 8487996 & Yes \\
3 & 8820786 & 8821159 & Yes \\
3 & 8884830 & 8887709 & Yes \\
3 & 8950320 & 8954906 & Yes \\
3 & 9088715 & 9093202 & Yes \\
3 & 9681452 & 9681634 & Yes \\
4 & 1186917 & 1188829 & Yes \\
4 & 13241336 & 13242118 & Yes \\
4 & 15552304 & 15553023 & No \\
4 & 15663794 & 15666868 & Yes \\
4 & 16043571 & 16043673 & No \\
4 & 18193659 & 18194827 & No \\
4 & 18673427 & 18675156 & Yes \\
4 & 2023060 & 2028629 & Yes \\
4 & 20409220 & 20411134 & Yes \\
4 & 20485903 & 20487331 & No \\
4 & 20559041 & 20560656 & Yes \\
4 & 21424020 & 21428007 & Yes \\
4 & 21429925 & 21436347 & Yes \\
4 & 22760322 & 22770287 & Yes \\
4 & 23366420 & 23367313 & Yes \\
4 & 23607275 & 23608177 & Yes \\
4 & 23658033 & 23658366 & Yes \\
4 & 26177720 & 26178192 & Yes \\
4 & 266586 & 268681 & Yes \\
4 & 27011171 & 27012610 & Yes \\
4 & 28773101 & 28773775 & Yes \\
4 & 28797150 & 28798631 & Yes \\
4 & 3154223 & 3156822 & Yes \\
4 & 3787223 & 3792365 & Yes \\
4 & 4654986 & 4664367 & Yes \\
4 & 5615032 & 5620106 & Yes \\
4 & 5724571 & 5726351 & Yes \\
4 & 7924375 & 7924526 & No \\
4 & 7952062 & 7952972 & Yes \\
4 & 8486213 & 8489486 & Yes \\
5 & 218441 & 224383 & Yes \\
5 & 357041 & 357831 & Yes \\
5 & 631600 & 632724 & Yes \\
\hline
\end{tabular}
\begin{tablenotes}
\item[]*\textbf{P},PindelConfirmed
\end{tablenotes}
 \label{tab:confirmations1}

\end{threeparttable}

 \end{center}
 
\clearpage
\begin{center}
\begin{threeparttable}
\caption{Pac Bio Confirmations for line CY21B3}
\tiny
\begin{tabular}{cccc}
 Chromosome &  Start &Stop & Confirmed \\
\hline
0 & 11082344 & 11085513 & Yes \\
0 & 11454199 & 11454798 & Yes \\
0 & 1172484 & 1179048 & Yes \\
0 & 11791812 & 11792896 & Yes \\
0 & 11841757 & 11854748 & Yes \\
0 & 12544338 & 12544932 & Yes \\
0 & 13913653 & 13913789 & Yes \\
0 & 14602982 & 14605035 & Yes \\
0 & 14666251 & 14666591 & Yes \\
0 & 15944998 & 15948170 & Yes \\
0 & 1631349 & 1632283 & Yes \\
0 & 16389408 & 16389696 & Yes \\
0 & 16689283 & 16690706 & Yes \\
0 & 1895238 & 1897322 & Yes \\
0 & 19273842 & 19287114 & Yes \\
0 & 19275592 & 19288918 & Yes \\
0 & 20096795 & 20097291 & Yes \\
0 & 20848448 & 20861465 & Yes \\
0 & 21013871 & 21014444 & Yes \\
0 & 21629444 & 21649018 & Yes \\
0 & 2198623 & 2199007 & Yes \\
0 & 22634141 & 22643599 & Yes \\
0 & 23060739 & 23073112 & Yes \\
0 & 23296027 & 23298592 & Yes \\
0 & 2397145 & 2400994 & Yes \\
0 & 2540641 & 2541141 & Yes \\
0 & 26147 & 26547 & Yes \\
0 & 4843038 & 4844658 & Yes \\
0 & 6853202 & 6857398 & Yes \\
0 & 6884747 & 6887564 & Yes \\
0 & 8272090 & 8281797 & Yes \\
0 & 8280380 & 8281789 & Yes \\
0 & 833632 & 833787 & Yes \\
0 & 9245383 & 9245534 & Yes \\
1 & 10585970 & 10587591 & Yes \\
1 & 10873174 & 10876328 & Yes \\
1 & 115508 & 115741 & Yes \\
1 & 11616544 & 11627893 & Yes \\
1 & 11727945 & 11728382 & Yes \\
1 & 12540167 & 12540379 & Yes \\
1 & 12589873 & 12593820 & Yes \\
1 & 12770060 & 12770210 & Yes \\
1 & 13058912 & 13060325 & Yes \\
1 & 14060529 & 14065910 & Yes \\
1 & 146434 & 147628 & Yes \\
1 & 15118394 & 15122003 & Yes \\
1 & 15197583 & 15197769 & Yes \\
1 & 15412553 & 15414703 & Yes \\
1 & 17477743 & 17483758 & Yes \\
1 & 18562314 & 18563395 & Yes \\
1 & 1859793 & 1864418 & Yes \\
1 & 18911824 & 18912498 & Yes \\
1 & 20258194 & 20258833 & Yes \\
1 & 20585587 & 20586694 & Yes \\
1 & 20592453 & 20594586 & Yes \\
1 & 20701045 & 20702768 & Yes \\
1 & 20851838 & 20856752 & Yes \\
1 & 20867709 & 20868709 & Yes \\
1 & 21051596 & 21051807 & Yes \\
1 & 21069963 & 21070572 & Yes \\
1 & 21070137 & 21072585 & Yes \\
1 & 21762468 & 21778962 & Yes \\
1 & 21767680 & 21782352 & Yes \\
1 & 21860804 & 21864242 & Yes \\
1 & 21869589 & 21890488 & Yes \\
1 & 21869791 & 21882786 & Yes \\
1 & 21888859 & 21890541 & Yes \\
1 & 22076307 & 22081156 & Yes \\
1 & 22142495 & 22143242 & Yes \\
1 & 22183097 & 22188165 & Yes \\
1 & 22229672 & 22240590 & Yes \\
1 & 22250930 & 22252868 & Yes \\
1 & 2726172 & 2731718 & Yes \\
1 & 4450246 & 4457268 & Yes \\
1 & 4561989 & 4563943 & Yes \\
1 & 463976 & 465681 & Yes \\
1 & 4707565 & 4707730 & Yes \\
1 & 5823306 & 5823695 & Yes \\
1 & 617863 & 618163 & Yes \\
1 & 6924773 & 6926435 & Yes \\
1 & 7043543 & 7048586 & Yes \\
1 & 7051842 & 7052051 & Yes \\
1 & 8569299 & 8569585 & Yes \\
1 & 8985224 & 8985885 & Yes \\
1 & 9638666 & 9639796 & Yes \\
1 & 964546 & 964895 & Yes \\
1 & 966613 & 966984 & Yes \\
2 & 10455751 & 10459056 & Yes \\
2 & 10705351 & 10711729 & Yes \\
2 & 10880419 & 10881086 & Yes \\
2 & 11060164 & 11061595 & Yes \\
2 & 11199268 & 11201983 & Yes \\
2 & 11216791 & 11218480 & Yes \\
2 & 11522584 & 11523299 & Yes \\
2 & 1192252 & 1198186 & Yes \\
2 & 12175793 & 12177566 & Yes \\
2 & 126303 & 128688 & Yes \\
2 & 1267547 & 1269515 & Yes \\
2 & 1283153 & 1285342 & Yes \\
2 & 1298866 & 1302456 & Yes \\
2 & 13042582 & 13049000 & Yes \\
2 & 13363163 & 13365446 & Yes \\
2 & 14915735 & 14922064 & Yes \\
2 & 14921170 & 14923118 & Yes \\
2 & 15591344 & 15591787 & Yes \\
2 & 156663 & 160152 & Yes \\
2 & 16500301 & 16500424 & Yes \\
2 & 17247998 & 17250046 & Yes \\
2 & 17738237 & 17742990 & Yes \\
2 & 17738426 & 17739224 & Yes \\
2 & 18125382 & 18132084 & Yes \\
2 & 181342 & 188388 & Yes \\
2 & 18340872 & 18341767 & Yes \\
2 & 184295 & 191096 & Yes \\
2 & 19236665 & 19238004 & Yes \\
2 & 20231452 & 20233075 & Yes \\
2 & 20346896 & 20349545 & Yes \\
2 & 20556535 & 20557016 & Yes \\
2 & 20677934 & 20678137 & Yes \\
2 & 223648 & 228167 & Yes \\
2 & 3566713 & 3567064 & Yes \\
2 & 363102 & 367650 & Yes \\
2 & 408041 & 414129 & Yes \\
2 & 4493045 & 4496695 & Yes \\
2 & 5069393 & 5069967 & No \\
2 & 5266448 & 5267383 & No \\
2 & 5347302 & 5349788 & Yes \\
2 & 543979 & 547207 & Yes \\
2 & 550564 & 555698 & Yes \\
2 & 5986750 & 5988343 & Yes \\
2 & 624166 & 625665 & Yes \\
2 & 6618311 & 6618962 & Yes \\
2 & 664616 & 665800 & Yes \\
2 & 6888816 & 6889491 & Yes \\
2 & 7486324 & 7489683 & Yes \\
2 & 7499439 & 7501545 & Yes \\
2 & 79391 & 104308 & Yes \\
2 & 8432422 & 8439919 & Yes \\
2 & 8627195 & 8631730 & Yes \\
2 & 8693878 & 8697950 & Yes \\
2 & 898282 & 901648 & Yes \\
2 & 901994 & 911580 & Yes \\
2 & 9371320 & 9371618 & Yes \\
2 & 9718894 & 9722579 & Yes \\
3 & 10097943 & 10098401 & Yes \\
3 & 10460172 & 10460672 & Yes \\
3 & 10796998 & 10797687 & Yes \\
3 & 11399149 & 11401565 & Yes \\
3 & 11401395 & 11401551 & Yes \\
3 & 13545130 & 13546858 & Yes \\
3 & 13959936 & 13960145 & Yes \\
3 & 14759218 & 14759582 & Yes \\
3 & 15899218 & 15899373 & Yes \\
3 & 15958742 & 15959096 & Yes \\
3 & 1616894 & 1617449 & Yes \\
3 & 16990151 & 16990245 & Yes \\
3 & 17554023 & 17554145 & Yes \\
3 & 17844417 & 17845634 & Yes \\
3 & 18352108 & 18352385 & Yes \\
3 & 18364150 & 18364287 & Yes \\
3 & 18481444 & 18482823 & Yes \\
3 & 18803792 & 18803955 & Yes \\
3 & 18808010 & 18808880 & Yes \\
3 & 18810158 & 18810616 & Yes \\
3 & 19154275 & 19154340 & Yes \\
3 & 20640778 & 20646886 & Yes \\
3 & 20761443 & 20768078 & Yes \\
3 & 21247532 & 21253286 & Yes \\
3 & 21252863 & 21277771 & Yes \\
3 & 21269788 & 21269996 & Yes \\
3 & 21426382 & 21432450 & Yes \\
3 & 2263061 & 2263383 & Yes \\
3 & 2538959 & 2540881 & Yes \\
3 & 2808 & 3095 & Yes \\
3 & 2911420 & 2911676 & Yes \\
3 & 3429367 & 3429542 & Yes \\
3 & 5076711 & 5077409 & Yes \\
3 & 6027171 & 6028326 & Yes \\
3 & 6457644 & 6459528 & Yes \\
3 & 6844781 & 6845813 & Yes \\
3 & 7531990 & 7532616 & Yes \\
3 & 8318145 & 8319291 & Yes \\
3 & 8783493 & 8784480 & Yes \\
3 & 8880918 & 8884990 & Yes \\
3 & 8950320 & 8954906 & Yes \\
3 & 9092346 & 9093590 & Yes \\
3 & 9681452 & 9681634 & Yes \\
4 & 10734970 & 10739334 & Yes \\
4 & 12277325 & 12278940 & Yes \\
4 & 12581548 & 12584840 & Yes \\
4 & 12761596 & 12766053 & Yes \\
4 & 12761603 & 12764289 & Yes \\
4 & 17211800 & 17212227 & Yes \\
4 & 18267617 & 18268749 & Yes \\
4 & 18698235 & 18698511 & Yes \\
4 & 2023060 & 2028629 & Yes \\
4 & 20559041 & 20560656 & Yes \\
4 & 21424020 & 21428007 & Yes \\
4 & 22065875 & 22066346 & Yes \\
4 & 23173632 & 23174079 & Yes \\
4 & 23189294 & 23190180 & Yes \\
4 & 23366731 & 23366855 & Yes \\
4 & 25034917 & 25051968 & Yes \\
4 & 25036642 & 25044043 & Yes \\
4 & 25372683 & 25379092 & Yes \\
4 & 26016459 & 26016872 & Yes \\
4 & 26042644 & 26043641 & Yes \\
4 & 265441 & 269975 & Yes \\
4 & 26908959 & 26909533 & Yes \\
4 & 27377585 & 27377782 & Yes \\
4 & 28797150 & 28798631 & Yes \\
4 & 3575739 & 3578766 & Yes \\
4 & 3787223 & 3792365 & Yes \\
4 & 4398247 & 4408273 & Yes \\
4 & 4654986 & 4664367 & Yes \\
4 & 5615032 & 5620106 & Yes \\
4 & 5724571 & 5726351 & Yes \\
4 & 6410021 & 6415561 & Yes \\
4 & 7107602 & 7112387 & Yes \\
4 & 7811211 & 7812300 & Yes \\
4 & 7927779 & 7928259 & Yes \\
4 & 7927779 & 7930632 & Yes \\
4 & 7952136 & 7953645 & Yes \\
5 & 218441 & 224383 & Yes \\
\hline
\end{tabular}
\begin{tablenotes}
\item[]*\textbf{P},PindelConfirmed
\end{tablenotes}
 \label{tab:confirmations2}

\end{threeparttable}
\end{center}

\clearpage
\begin{center}
\begin{threeparttable}
\caption{Pac Bio confirmations for line NY66-2}
\tiny
\begin{tabular}{cccc}
 Chromosome & Start & Stop & Confirmed \\
\hline
0 & 11841757 & 11854748 & Yes \\
0 & 12173462 & 12175684 & No \\
0 & 12894471 & 12894671 & Yes \\
0 & 13385592 & 13386716 & Yes \\
0 & 1341315 & 1341538 & Yes \\
0 & 15023729 & 15026407 & Yes \\
0 & 1631349 & 1632283 & Yes \\
0 & 16520655 & 16536465 & Yes \\
0 & 16525247 & 16536468 & Yes \\
0 & 18450050 & 18452705 & Yes \\
0 & 22160922 & 22173382 & Yes \\
0 & 4748069 & 4750627 & Yes \\
0 & 4779400 & 4780127 & Yes \\
0 & 6615959 & 6616840 & Yes \\
0 & 8234774 & 8235082 & Yes \\
0 & 8269178 & 8271229 & Yes \\
0 & 8735178 & 8735793 & Yes \\
1 & 10585970 & 10587591 & Yes \\
1 & 12184365 & 12184462 & Yes \\
1 & 12589873 & 12593820 & Yes \\
1 & 13575223 & 13575590 & Yes \\
1 & 13658567 & 13660529 & Yes \\
1 & 14059272 & 14059723 & Yes \\
1 & 15037862 & 15038705 & Yes \\
1 & 16173723 & 16173986 & Yes \\
1 & 1689506 & 1689665 & Yes \\
1 & 19375059 & 19376388 & Yes \\
1 & 19481376 & 19484185 & Yes \\
1 & 19846732 & 19846992 & Yes \\
1 & 20405582 & 20408626 & Yes \\
1 & 20585587 & 20586694 & Yes \\
1 & 20867709 & 20868709 & Yes \\
1 & 21138581 & 21141816 & Yes \\
1 & 21392066 & 21396534 & Yes \\
1 & 21860804 & 21864242 & Yes \\
1 & 21981789 & 21983449 & Yes \\
1 & 22142495 & 22143242 & Yes \\
1 & 22183097 & 22188165 & Yes \\
1 & 22202637 & 22205208 & Yes \\
1 & 22229672 & 22240590 & Yes \\
1 & 2229899 & 2234096 & Yes \\
1 & 2420441 & 2420599 & Yes \\
1 & 5104537 & 5104808 & No \\
1 & 5725980 & 5726127 & No \\
1 & 7051842 & 7052051 & Yes \\
2 & 10699218 & 10701733 & Yes \\
2 & 10705351 & 10711729 & Yes \\
2 & 11199268 & 11201983 & Yes \\
2 & 11275346 & 11277426 & Yes \\
2 & 1131987 & 1133889 & Yes \\
2 & 11522584 & 11523299 & Yes \\
2 & 1192252 & 1198186 & Yes \\
2 & 126303 & 128688 & Yes \\
2 & 12873611 & 12874020 & Yes \\
2 & 1298866 & 1302456 & Yes \\
2 & 13593056 & 13597666 & Yes \\
2 & 15447621 & 15450093 & Yes \\
2 & 17738237 & 17742990 & Yes \\
2 & 189694 & 195893 & Yes \\
2 & 20384228 & 20385080 & Yes \\
2 & 21031498 & 21031658 & Yes \\
2 & 2450808 & 2456264 & Yes \\
2 & 2456185 & 2468412 & Yes \\
2 & 3530693 & 3530879 & Yes \\
2 & 3600589 & 3603993 & Yes \\
2 & 4871836 & 4872286 & No \\
2 & 550564 & 555698 & Yes \\
2 & 664616 & 665800 & Yes \\
2 & 6990941 & 6992414 & Yes \\
2 & 8627195 & 8631730 & Yes \\
2 & 8693878 & 8697950 & Yes \\
2 & 8762236 & 8764448 & Yes \\
2 & 898282 & 901648 & Yes \\
2 & 9302688 & 9307472 & Yes \\
2 & 9718894 & 9722579 & Yes \\
3 & 10060151 & 10060351 & Yes \\
3 & 11042137 & 11042331 & Yes \\
3 & 11399149 & 11401565 & Yes \\
3 & 11399250 & 11399374 & Yes \\
3 & 11401395 & 11401551 & Yes \\
3 & 12994638 & 12995090 & Yes \\
3 & 14420131 & 14420863 & Yes \\
3 & 15977640 & 15977783 & Yes \\
3 & 16469587 & 16470148 & Yes \\
3 & 18810158 & 18810616 & Yes \\
3 & 19027974 & 19028125 & Yes \\
3 & 1914150 & 1915867 & Yes \\
3 & 19466157 & 19466283 & Yes \\
3 & 19934644 & 19934827 & Yes \\
3 & 20640778 & 20646886 & Yes \\
3 & 20676848 & 20686617 & Yes \\
3 & 21426382 & 21432450 & Yes \\
3 & 291478 & 293921 & Yes \\
3 & 3429367 & 3429542 & Yes \\
3 & 3720837 & 3721117 & Yes \\
3 & 6027171 & 6028326 & Yes \\
3 & 6034154 & 6034546 & Yes \\
3 & 63087 & 65284 & Yes \\
3 & 6686813 & 6687881 & Yes \\
3 & 6870847 & 6871139 & Yes \\
3 & 6954658 & 6955050 & Yes \\
3 & 7163081 & 7187882 & Yes \\
3 & 7609261 & 7613569 & Yes \\
3 & 8318145 & 8319291 & Yes \\
3 & 8767079 & 8767219 & Yes \\
3 & 8950320 & 8954906 & Yes \\
3 & 9088715 & 9093202 & Yes \\
3 & 9681452 & 9681634 & Yes \\
4 & 10546945 & 10548114 & No \\
4 & 12954570 & 12954778 & Yes \\
4 & 14703209 & 14705506 & Yes \\
4 & 16597197 & 16599213 & Yes \\
4 & 17211800 & 17212227 & Yes \\
4 & 18267617 & 18268749 & Yes \\
4 & 19721096 & 19721470 & Yes \\
4 & 20679513 & 20679786 & Yes \\
4 & 21429925 & 21436347 & Yes \\
4 & 22065875 & 22066346 & Yes \\
4 & 24264897 & 24268002 & Yes \\
4 & 25034917 & 25051968 & Yes \\
4 & 25372683 & 25379092 & Yes \\
4 & 26969738 & 26971104 & Yes \\
4 & 27011171 & 27012610 & Yes \\
4 & 27156036 & 27156149 & Yes \\
4 & 27861882 & 27865392 & Yes \\
4 & 27982410 & 27982551 & Yes \\
4 & 28728373 & 28728972 & Yes \\
4 & 28797150 & 28798631 & Yes \\
4 & 456693 & 474667 & Yes \\
4 & 6706787 & 6720136 & Yes \\
4 & 7832431 & 7833298 & No \\
4 & 9234367 & 9234559 & Yes \\
5 & 181016 & 183366 & Yes \\
5 & 218441 & 224383 & Yes \\
\hline
\end{tabular}
\begin{tablenotes}
\item[]*\textbf{P},PindelConfirmed
\end{tablenotes}
 \label{tab:confirmations3}
 \end{threeparttable}
\end{center}


\clearpage
\begin{center}
\begin{threeparttable}
\caption{Pac Bio confirmations for line NY73}
\tiny
\begin{tabular}{cccc}
 Chromosome & Start & Stop & Confirmed \\
\hline
0 & 10560993 & 10561420 & Yes \\
0 & 11082344 & 11085513 & Yes \\
0 & 11612604 & 11613733 & Yes \\
0 & 1360250 & 1360761 & Yes \\
0 & 13803259 & 13804705 & Yes \\
0 & 14253136 & 14253504 & Yes \\
0 & 15042152 & 15042820 & Yes \\
0 & 15139699 & 15140490 & Yes \\
0 & 15792832 & 15793011 & Yes \\
0 & 15944832 & 15946907 & Yes \\
0 & 1631349 & 1632283 & Yes \\
0 & 16689283 & 16690706 & Yes \\
0 & 18741929 & 18746697 & Yes \\
0 & 2242665 & 2243279 & Yes \\
0 & 23446196 & 23449515 & Yes \\
0 & 282949 & 286511 & Yes \\
0 & 4652609 & 4652847 & No \\
0 & 4779400 & 4780127 & Yes \\
0 & 6853202 & 6857398 & Yes \\
0 & 8280380 & 8281789 & Yes \\
0 & 8645355 & 8645729 & Yes \\
1 & 13658567 & 13660529 & No \\
1 & 1859793 & 1864418 & Yes \\
1 & 19375059 & 19376388 & Yes \\
1 & 20187122 & 20187297 & No \\
1 & 20361093 & 20361828 & Yes \\
1 & 20585587 & 20586694 & Yes \\
1 & 20625603 & 20627567 & Yes \\
1 & 20633316 & 20634367 & Yes \\
1 & 20867709 & 20868709 & Yes \\
1 & 21860804 & 21864242 & Yes \\
1 & 21888859 & 21890541 & Yes \\
1 & 22142495 & 22143242 & Yes \\
1 & 22217615 & 22221738 & Yes \\
1 & 22229672 & 22240590 & Yes \\
1 & 4561989 & 4563943 & Yes \\
1 & 481149 & 481530 & No \\
1 & 7051842 & 7052051 & Yes \\
1 & 9635539 & 9643235 & Yes \\
1 & 966613 & 966984 & Yes \\
2 & 11199268 & 11201983 & Yes \\
2 & 11522584 & 11523299 & Yes \\
2 & 1220523 & 1223522 & Yes \\
2 & 1254226 & 1254666 & Yes \\
2 & 126303 & 128688 & Yes \\
2 & 13052601 & 13054893 & Yes \\
2 & 18125382 & 18132084 & Yes \\
2 & 187210 & 187430 & Yes \\
2 & 20346896 & 20349545 & Yes \\
2 & 20547562 & 20548621 & No \\
2 & 20556535 & 20557016 & Yes \\
2 & 21100065 & 21101659 & Yes \\
2 & 2450808 & 2456264 & Yes \\
2 & 2456185 & 2468412 & Yes \\
2 & 543979 & 547207 & Yes \\
2 & 550564 & 555698 & Yes \\
2 & 5880254 & 5883193 & Yes \\
2 & 5986750 & 5988343 & Yes \\
2 & 6887339 & 6887770 & Yes \\
2 & 831842 & 836470 & Yes \\
2 & 8627195 & 8631730 & Yes \\
2 & 8693878 & 8697950 & Yes \\
2 & 898282 & 901648 & Yes \\
2 & 9718894 & 9722579 & Yes \\
3 & 12616185 & 12616299 & Yes \\
3 & 12994638 & 12995090 & Yes \\
3 & 13253505 & 13253606 & Yes \\
3 & 14183464 & 14183685 & Yes \\
3 & 15375448 & 15375633 & No \\
3 & 17439344 & 17439758 & No \\
3 & 18352108 & 18352385 & Yes \\
3 & 18633734 & 18634217 & Yes \\
3 & 18729973 & 18730230 & Yes \\
3 & 19810217 & 19810349 & Yes \\
3 & 20074771 & 20074908 & No \\
3 & 20761443 & 20768078 & Yes \\
3 & 21252863 & 21277771 & Yes \\
3 & 2263061 & 2263383 & Yes \\
3 & 2911420 & 2911676 & Yes \\
3 & 291478 & 293921 & Yes \\
3 & 3050809 & 3051184 & Yes \\
3 & 6027171 & 6028326 & Yes \\
3 & 6034154 & 6034546 & Yes \\
3 & 6694567 & 6695032 & Yes \\
3 & 6979162 & 6979796 & Yes \\
4 & 12685410 & 12688723 & Yes \\
4 & 17035562 & 17038719 & Yes \\
4 & 17211800 & 17212227 & Yes \\
4 & 17786235 & 17790099 & Yes \\
4 & 18267617 & 18268749 & Yes \\
4 & 18382396 & 18384823 & Yes \\
4 & 22065875 & 22066346 & Yes \\
4 & 23908007 & 23911565 & Yes \\
4 & 25372683 & 25379092 & Yes \\
4 & 26616440 & 26618338 & Yes \\
4 & 26908959 & 26909533 & Yes \\
4 & 28773101 & 28773775 & No \\
4 & 28797150 & 28798631 & Yes \\
4 & 4654986 & 4664367 & Yes \\
4 & 5928252 & 5928605 & Yes \\
\hline
\end{tabular}
\begin{tablenotes}
\item[]*\textbf{P},PindelConfirmed
\end{tablenotes}
 \label{tab:confirmations4}
\end{threeparttable}
\end{center}

